Conic Mixed-Binary Sets: Convex Hull Characterizations and Applications

We consider a general conic mixed-binary set where each homogeneous conic constraint $j$ involves an affine function of independent continuous variables and an epigraph variable associated with a nonnegative function, $f_j$, of common binary variables. Sets of this form naturally arise as substructures in a number of applications including mean-risk optimization, chance-constrained problems, portfolio optimization, lot-sizing and scheduling, fractional programming, variants of the best subset selection problem, a class of sparse semidefinite programs, and distributionally robust chance-constrained programs. We give a convex hull description of this set that relies on simultaneous characterization of the epigraphs of $f_j$'s, which is easy to do when all functions $f_j$'s are submodular. Our result unifies and generalizes an existing result in two important directions. First, it considers \emph{multiple general convex cone} constraints instead of a single second-order cone type constraint. Second, it takes \emph{arbitrary nonnegative functions} instead of a specific submodular function obtained from the square root of an affine function. We close by demonstrating the applicability of our results in the context of a number of problem classes.

==> fatma-macros.tex <==
\def\crd{\color{red}}
\def\cbl{\color{blue}}
\def\cgr{\color{green}}
\def\cmg{\color{magenta}}
\def\ccy{\color{cyan}}
\def\cye{\color{yellow}}
\definecolor{gold}{rgb}{0.85,0.65,0}

\newcommand{\floor}[1]{\ensuremath{\left\lfloor #1 \right\rfloor}}
\newcommand{\ceil}[1]{\ensuremath{\left\lceil #1 \right\rceil}}
\newcommand{\abs}[1]{\ensuremath{\left\lvert #1 \right\rvert}}
\DeclareMathOperator{\poly}{poly}
\newcommand{\by}{\times}
 
\newcommand{\norm}[1]{\ensuremath{\left\lVert #1 \right\rVert}}
\newcommand{\ip}[1]{\ensuremath{\left\langle #1 \right\rangle}}
\newcommand{\grad}{\ensuremath{\nabla}}

\let\oldemptyset\emptyset
\let\emptyset\varnothing
\newcommand{\set}[1]{\left\{#1\right\}}

\newcommand{\mb}{\bm}
\newcommand{\bs}{\boldsymbol}
\newcommand{\bb}{\mathbb}
\newcommand{\mf}{\mathfrak}

\def\A{{\mathbb{A}}}
\def\B{{\mathbb{B}}}
\def\C{{\mathbb{C}}}
\def\D{{\mathbb{D}}}
\def\F{{\mathbb{F}}}
\def\G{{\mathbb{G}}}
\def\H{{\mathbb{H}}}
\def\I{{\mathbb{I}}}
\def\J{{\mathbb{J}}}
\def\K{{\mathbb{K}}}
\def\L{{\mathbb{L}}}
\def\M{{\mathbb{M}}}
\def\N{{\mathbb{N}}}
\def\O{{\mathbb{O}}}
\def\P{{\mathbb{P}}}
\def\Q{{\mathbb{Q}}}
\def\R{{\mathbb{R}}}
\def\S{{\mathbb{S}}}
\def\T{{\mathbb{T}}}
\def\U{{\mathbb{U}}}
\def\V{{\mathbb{V}}}
\def\W{{\mathbb{W}}}
\def\X{{\mathbb{X}}}
\def\Y{{\mathbb{Y}}}
\def\Z{{\mathbb{Z}}}

\def\bA{{\bm{A}}}
\def\bB{{\bm{B}}}
\def\bC{{\bm{C}}}
\def\bD{{\bm{D}}}
\def\bE{{\bm{E}}}
\def\bF{{\bm{F}}}
\def\bG{{\bm{G}}}
\def\bH{{\bm{H}}}
\def\bI{{\bm{I}}}
\def\bJ{{\bm{J}}}
\def\bK{{\bm{K}}}
\def\bL{{\bm{L}}}
\def\bM{{\bm{M}}}
\def\bN{{\bm{N}}}
\def\bO{{\bm{O}}}
\def\bP{{\bm{P}}}
\def\bQ{{\bm{Q}}}
\def\bR{{\bm{R}}}
\def\bS{{\bm{S}}}
\def\bT{{\bm{T}}}
\def\bU{{\bm{U}}}
\def\bV{{\bm{V}}}
\def\bW{{\bm{W}}}
\def\bX{{\bm{X}}}
\def\bY{{\bm{Y}}}
\def\bZ{{\bm{Z}}}

\def\cA{{\cal A}}
\def\cB{{\cal B}}
\def\cC{{\cal C}}
\def\cD{{\cal D}}
\def\cE{{\cal E}}
\def\cF{{\cal F}}
\def\cG{{\cal G}}
\def\cH{{\cal H}}
\def\cI{{\cal I}}
\def\cJ{{\cal J}}
\def\cK{{\cal K}}
\def\cL{{\cal L}}
\def\cM{{\cal M}}
\def\cN{{\cal N}}
\def\cO{{\cal O}}
\def\cP{{\cal P}}
\def\cQ{{\cal Q}}
\def\cR{{\cal R}}
\def\cS{{\cal S}}
\def\cT{{\cal T}}
\def\cU{{\cal U}}
\def\cV{{\cal V}}
\def\cW{{\cal W}}
\def\cX{{\cal X}}
\def\cY{{\cal Y}}
\def\cZ{{\cal Z}}

\def\mones{{\bm{1}}}

\DeclareMathOperator{\Opt}{Opt}

\DeclareMathOperator{\rank}{rank}
\DeclareMathOperator{\Diag}{Diag}
\DeclareMathOperator{\diag}{diag}
\DeclareMathOperator{\tr}{tr}
\DeclareMathOperator{\col}{col}
\DeclareMathOperator{\row}{row}
\DeclareMathOperator{\nulll}{null}
\DeclareMathOperator{\Image}{Im}
\DeclareMathOperator{\range}{range}
\newenvironment{smallpmatrix}
{\left(\begin{smallmatrix}}
{\end{smallmatrix}\right)}


\DeclareMathOperator*{\E}{\mathbb{E}}
\DeclareMathOperator{\Var}{var}

\DeclareMathOperator{\codim}{codim}
\DeclareMathOperator{\aff}{aff}
\DeclareMathOperator{\spann}{span}
\DeclareMathOperator{\inter}{int}
\DeclareMathOperator{\rint}{rint}
\DeclareMathOperator{\cl}{cl}
\DeclareMathOperator{\bd}{bd}
\DeclareMathOperator{\rbd}{rbd}

\DeclareMathOperator{\dom}{dom}
\DeclareMathOperator{\Dom}{dom}
\DeclareMathOperator{\epi}{epi}
\DeclareMathOperator{\Epi}{epi}
\DeclareMathOperator{\hyp}{hyp}
\DeclareMathOperator{\Hyp}{hyp}

\DeclareMathOperator{\conv}{conv}
\DeclareMathOperator{\cone}{cone}
\DeclareMathOperator{\clconv}{clconv}
\DeclareMathOperator{\clcone}{clcone}
\def\extr{{\mathop{\rm extr}}}
\DeclareMathOperator{\rec}{rec}
\DeclareMathOperator{\apex}{apex}

\newcommand{\intset}[1]{\left\llbracket #1 \right\rrbracket}

\DeclareMathOperator{\Sym}{Sym}

\DeclareMathOperator{\Proj}{Proj}


\newcommand{\obj}{\textup{obj}}
\newcommand{\gobj}{\gamma_\obj}
\newcommand{\qobj}{q_\obj}
\newcommand{\Mobj}{M_\obj}


\newcommand{\face}{\triangleleft}
\newcommand{\faceeq}{\trianglelefteq}
\newcommand{\one}{{(1)}}
\newcommand{\onetop}{{(1)\top}}
\newcommand{\ones}{{\bm{1}}}
\newcommand{\two}{{(2)}}
\newcommand{\twotop}{{(2)\top}}

\newcommand{\SDP}{\textup{SDP}}
\newcommand{\RLT}{\textup{RLT}}
\newcommand{\conic}{\textup{conic}}
\def\Le{{\mathbb{L}}}
\def\Se{{\mathbb{S}}}

\DeclareMathOperator{\supp}{supp}
\DeclareMathOperator{\zeros}{zeros}
\newcommand{\aas}{\textit{a.a.s.}}
\newcommand{\ngoe}{\textup{NGOE}}
\newcommand{\nsc}{\textup{nsc}}
\newcommand{\esd}{\textup{ESD}}

\newcommand{\Sbar}{\overline{\cS}(\bm f, \cZ)}
\newcommand{\Fleq}{\cF_{\leq}(\bm f, \cZ)}
\newcommand{\Fgeq}{\cF_{\geq}(\bm f, \cZ)}
\newcommand{\x}{{\bm x}}
\newcommand{\z}{{\bm z}}
\newcommand{\y}{{\bm y}}
\newcommand{\f}{{\bm f}}
\newcommand{\e}{{\bm e}}
\renewcommand{\u}{{\bm u}}
\renewcommand{\v}{{\bm v}}
\renewcommand{\t}{{\bm t}}






